The Value of Compromising Strategic Intent in General Lotto Games

Resource allocation in adversarial environments is a fundamental challenge across various domains, from corporate competition to military strategy. This article examines the impact of compromising an opponent's strategic intent in the context of General Lotto games, a class of resource allocation problems. We consider a scenario where one player, termed the "Breaker", has access to partial information about their opponent's strategy through a binary sensor. This sensor reveals whether the opponent's allocated resources exceed a certain threshold. Our analysis provides a comprehensive characterization of equilibrium strategies and payoffs for both players under this information structure. Through numerical studies, we demonstrate that the information provided by the sensor can significantly improve the Breaker's performance.

==> introduction_kp.tex <==
% !TEX root = main.tex

% Need to talk about the need to get a competitive advantage.  Opportunities here are plentiful, such as expanding forces or acquiring information about an adversary.  The focus of this paper is..

In order to maximize chances of success, competitors seek to gain an edge over their opponents -- whether they are rival corporations, political candidates, or defenders and attackers of an infrastructure system. One can improve its competitive position by increasing its own capabilities through investing in better quality resources, diminishing the capabilities of opponents, forming cooperative alliances with others, or by acquiring information about the environment. Depending on the scenario and environmental conditions, some of these approaches may prove to be successful, while others may not. As a result, such strategic mechanisms are extensively studied in many different contexts with regards to decision-making in adversarial environments.

% Need to focus more on highlevel question, where CB and GL are just particular problem settings that we will study this in.

In this work, we are particularly interested in examining how acquired information about an opponent's plan of action can impact one's performance compared to a scenario where no such information is available. A representative example is the placement of intrusion detection systems for the purpose of improving security against cyber-attackers. More generally, a defender is capable of unveiling strategic behaviors of potential adversaries, and utilize this timely information to respond accordingly. In other words, the defender has information-gathering mechanisms in place that can compromise an attacker's strategic intent. Figure \ref{fig:diagram} provides an illustration.


The importance of timely interception of information about an attacker's planned behaviors cannot be overstated. Numerous historical events occurred because of the successful decryption of encoded messages: cracking the Enigma in WWII, and the execution of Mary, Queen of Scots in 1587 upon decoding her plans against Elizabeth I. Information acquisition is arguably even more important today, as the security of computer networks and infrastructures relies on gathering up-to-date intelligence.





% % % % % % % % % % % % % % % % % % % % 


The interconnected nature of modern network systems creates many new vulnerabilities for adversarial actors to exploit. Consequently, the allocation of security assets across system components is an increasingly important strategic consideration that needs to be incorporated in security policies. A critical aspect tied into this is the information asymmetry that may arise between defenders and adversaries.  Knowledge about an adversary’s plan of action and intent can potentially lead to significant improvements in security. 


The emerging framework of Colonel Blotto games \cite{Roberson_2006,kovenock2021generalizations} is well-tuned to study strategic resource allocation in large-scale systems, and has gained widespread uses \cite{Schwartz_2014,Shahrivar_2014,Ferdowsi_2020,Shishika_2021}. In a Blotto game, two competing players allocate their limited resources over multiple valuable contests. A player secures a contest by allocating more resources than the opponent, and the objective is to maximize the value accrued by securing individual contests. 

However, it is well-known that solutions to Blotto games are often prohibitively challenging to obtain. For this reason, the popular variant known as \emph{General Lotto games} has been preferred in recent years because it is much more amenable to analysis. General Lotto games have effectively extended the Blotto framework along many dimensions, e.g. to networked systems \cite{Kovenock_2018,aghajanNetworkedCDC2022}, multiple competitors \cite{Kovenock_2012,Gupta_2014a}, and incomplete information \cite{Paarporn_2019}.



In this work, we consider  informational asymmetry in the context of General Lotto games where information about an opponent's  strategy can be exploited. We examine a scenario where two players, $A$ and $B$,  compete over a single valuable contest. One of the players, say $B$, receives information from a sensor before competition takes place. The sensor is specified by a fixed threshold $\tau \geq 0$, and it signals to player $B$ whether the amount of  player $A$'s resources allocated to the contest was above or below the threshold. Once the sensor sends the signal, player $A$ is unable to alter its allocation. On the other hand, player $B$ is able to select its strategy based on the signal it received. We term this scenario as the General Lotto game with binary information. 

% In order to analyze this scenario, 
\subsection{Contributions}
The contributions of this work are summarized below.
\begin{enumerate}
    \item Full analytical characterization of the equilibrium strategies and payoffs to both players in the General Lotto game with binary information. The results are general for any threshold $\tau$ and any player resource budgets $X_A$ and $X_B$.
    \item Derivation of the optimal threshold selection $\tau^*$ for player $B$. This selection maximizes its equilibrium payoff in the General Lotto game with binary information. \gdg{I thought that we were not including this results for the conference version. I just remove them from the document.}
    \item Numerical study that suggest a threshold sensor can provide significant performance improvements in comparison to having no sensor.
\end{enumerate}
In order to establish the main contribution, item 1, we need to characterize optimal strategies in two different sub-games -- the one where the sensor signals below the threshold, and the one where the sensor signals above the threshold. Some of the analysis of these sub-games are novel contributions to the literature as well.

\subsection{Related literature}
Colonel Blotto and General Lotto games with incomplete information have received attention in recent years \cite{Adamo_2009,Kovenock_2011,Paarporn_2019,lotto:uncertain,paarporn2023strategically,Ewerhart_2021}. These papers primarily consider scenarios where players hold uncertainty about the underlying environmental parameters, e.g. opponent's budgets or contest valuations. Our present work differs in that the uncertainty stems from a player's implemented strategy (i.e. a sample from its mixed strategy), rather than from the uncertainty about a fixed parameter.

Our present work is closest to the paper \cite{sensor}, which considered a similar setup in the context of Colonel Blotto games. There, the authors modeled threshold sensors over multiple contests, where the results pertaining to equilibrium characterizations were primarily derived numerically. In our work, we provide full analytical characterizations of equilibria in the General Lotto game. Another simmilar work is the paper \cite{brethouwer2024general}, which studied a General Lotto game with a different type of sensor that sometimes provides information about the exact amount of allocated resources.
